Faster Approximation Schemes and Parameterized Algorithms on H-Minor-Free and Odd-Minor-Free Graphs

We improve the running time of the general algorithmic technique known as Baker's approach (1994) on H-minor-free graphs from O(n^{f(|H|)}) to O(f(|H|) n^{O(1)}). The numerous applications include e.g. a 2-approximation for coloring and PTASes for various problems such as dominating set and max-cut, where we obtain similar improvements. On classes of odd-minor-free graphs, which have gained significant attention in recent time, we obtain a similar acceleration for a variant of the structural decomposition theorem proved by Demaine et al. (2010). We use these algorithms to derive faster 2-approximations; furthermore, we present the first PTASes and subexponential FPT-algorithms for independent set and vertex cover on these graph classes using a novel dynamic programming technique. We also introduce a technique to derive (nearly) subexponential parameterized algorithms on H-minor-free graphs. Our technique applies, in particular, to problems such as Steiner tree, (directed) subgraph with a property, (directed) longest path, and (connected/independent) dominating set, on some or all proper minor-closed graph classes. We obtain as a corollary that all problems with a minor-monotone subexponential kernel and amenable to our technique can be solved in subexponential FPT-time on H-minor free graphs. This results in a general methodology for subexponential parameterized algorithms outside the framework of bidimensionality.

==> conclusion.tex <==

\section{Conclusion}
\label{sect:conclusion}

We significantly accelerated one of the main tools in PTAS design --
namely, Baker's decomposition -- on all proper minor-closed graph
classes, thereby obtaining the improvement for all the applications of
this tool. We showed similar results for odd-minor-free graphs and
obtained the first PTAS and subexponential $\fpt$-algorithms for
$\vrtcover$ and $\indset$ on these graph classes. Based on Baker's
approach, we also introduced the new technique of Guess \& Conquer for
designing (nearly) subexponential $\fpt$-algorithms on these graph
classes. We improved the best known $\fpt$-algorithms for $\steiner$
and {\sc directed $k$-$\ppath$} that were previously only known to be
in $\ept$ even on planar / apex-minor-free graphs. We actually
conjecture that these problems are in $\subept$ on $H$-minor-free
graphs and repeat this as an important open question for future work.


==> intro.tex <==
\section{Introduction}
\label{sec:introduction}

One of the most seminal results in algorithmic graph theory is
arguably Baker's approach~\cite{Baker94} for designing polynomial-time
approximation schemes (PTAS) for a wide range of problems on planar
graphs. Ever since its discovery, it has been applied and generalized
in various ways, see
e.g.~\cite{Eppstein00-DT,FrickGrohe01,Grohe03,AlberFN04,Klein05-TSP,DemaineHK05,DemaineHM07,BorradaileKM09}. The
essence of the idea is the following: for any given $t$, one can
partition a planar graph into $t$ parts, so that removing any one of
the parts results in a graph of bounded treewidth. Now, to obtain a
PTAS, we observe that if $t$ is appropriately chosen, there must exist
a part that contains at most an $\epsilon$-fraction of an optimal
solution; this can often be combined with the solution in the
remainder of the graph to obtain a $(1+\epsilon)$-approximation.

$H$-minor-free graphs, i.e.\ proper graph classes that are closed
under building minors, have gained significant attention in the past
two decades, especially due to Robertson and Seymour's graph minor
theory, one of the deepest and most far-reaching theories in discrete
mathematics in the past few decades. These classes include, e.g.\
planar graphs, bounded-genus graphs, linklessly embeddable graphs and
apex graphs. Using the deep Robertson-Seymour (RS-) decomposition
theorem~\cite{GraphMinors16}, Grohe~\cite{Grohe03} generalized Baker's
technique to $H$-minor-free graphs and Demaine et
al.~\cite{DemaineHK05} showed the partitioning theorem mentioned above
for all these graph classes. However, both their methods result in
algorithms with running time $\Oof(n^{f(|H|)})$, for some computable
function $f$; since $H$ is assumed to be fixed, this is considered
polynomial.

\usec{Improving Baker's Decomposition} We provide the first algorithm
for Baker's decomposition running in time $\Oof(g(|H|) \poly)$, for
some computable function $g$. This is a significant acceleration of
the previous results, especially considering the fact that the
constants in graph minor theory, such as the functions $f,g$ above,
are usually huge. This immediately implies similar improvements on all
the consequences of this algorithm, especially \emph{all} the generic
approximation algorithms and schemes in~\cite{Grohe03,DemaineHK05} and
Baker's original problems~\cite{Baker94}. In particular, we obtain the
first $2$-approximation for $\coloring$ $H$-minor-free graphs in the
given time bound and the first PTAS for $\indset$, $\mincolorsum$,
$\maxcut$, $\maxPmatching$, and $\domset$ on these graph classes while
avoiding $|H|$ in the exponent of $n$ in their running time. Our main
idea is derived from Dawar et al.'s approach~\cite{DawarGK07} of
finding a certain tree decomposition of $H$-minor-free graphs that is
more tractable than the RS-decomposition.

\usec{Parameterized Complexity} In the language of parameterized
  complexity, our result above shows that partitioning $H$-minor-free
graphs in the described way is \emph{fixed-parameter tractable
  ($\fpt$)} when parameterized by $|H|$. In this framework, for a
given problem of size $n$ and parameter $k$, we are interested in
algorithms with a running time of $\Oof(f(k) \poly)$, where $f$ is
some computable function depending solely on $k$; we then say that the
problem at hand is in $\fpt$. The theory also provides negative evidence
that some problems are most likely not $\fpt$; we refer to the books
of Downey and Fellows~\cite{DowneyFellows99} and Flum and
Grohe~\cite{FlumGrohe06} for more background on parameterized
complexity.

Once a problem is shown to be $\fpt$, the challenge is to provide
algorithms that have the smallest dependence on the parameter $k$,
i.e.\ make the function $f$ in the running time as small as possible.
It is especially desirable to obtain \emph{subexponential} functions
and thus provide particularly fast algorithms.  Whereas this is often
not possible in general graphs, a plethora of results exist that show
the existence of such algorithms on restricted graph classes, such as
$H$-minor-free graphs.  Perhaps the most general technique to obtain
subexponential parameterized algorithms on these graph classes is the
theory of \emph{bidimensionality}~\cite{DemaineFHT05-JACM} that captures
almost all known results of this type on $H$-minor-free graphs.
Still, this theory does not apply to a number of prominent problems,
such as $\steiner$, $\cdomset$, and {\sc Directed $k$-\ppath}.

One way to show fixed-parameter tractability of a problem is to show
the existence of a \emph{kernel} for the problem, which is a
polynomial-time algorithm that transforms any instance into an
equivalent instance whose size is bounded by a function $g$ solely
dependent on $k$, called the \emph{size} of the kernel. Kernelization
can be seen as polynomial-time pre-processing with a quality guarantee
and has gained much theoretical importance in the recent years --
besides its natural practical importance. For an introduction to
kernels we refer to the survey by Guo and
Niedermeier~\cite{GuoNiedermeier07}.

\usec{Guess and Conquer} In this work, we provide a new framework,
that we call \emph{guess and conquer}, to obtain (nearly)
subexponential parameterized algorithms on $H$-minor-free graphs for
an abundant number of parameterized problems.  Whenever the problem at
hand admits a minor-monotone subexponential kernel, our method
results indeed in a subexponential algorithm; otherwise, we obtain an
algorithm with a running time $\subtimeA = \subtimeC$ which we call
\emph{nearly} subexponential.  Note that if $k = \Oof(\log n)$, our
running time is fully polynomial in the input and if $k = \omega(\log
n)$, it is subexponential $\fpt$ in $k$.  Hence, except for a ``small
range'' of possible parameter values, we have a subexponential $\fpt$
algorithm.  In fact, we show that the problems we consider, admit a
minor-monotone subexponential kernel on $H$-minor-free graphs if and
only if they admit a subexponential $\fpt$ algorithm on these graph
classes. Note that in general graphs, even a linear kernel results
only in an exponential $\fpt$-algorithm.

Our technique applies in particular to $\cdomset$ and $\steiner$ (at
least) in bounded-genus graphs and {\sc Directed $k$-\ppath} in all
$H$-minor-free graphs, none of which are known to admit subexponential
$\fpt$-algorithms in $H$-minor-free graphs; for the latter two, such
algorithms are not even known for planar graphs.

At the time of preparation of this paper, we became aware that Dorn et
al.~\cite{DornFLRS10} recently and independently obtained similar
nearly subexponential algorithms for some problems, albeit \emph{only
  on apex-minor-free} graphs -- whereas our techniques apply to
general $H$-minor-free graphs. The focus of their work is on directed
graph problems and in particular, they obtain a nearly
subexponential $\fpt$-algorithm for {\sc Directed $k$-\ppath} in
apex-minor-free graphs (furthermore, they obtain a number of
subexponential $\fpt$-algorithms for problems that we do not consider
in this work). The second method they present in their paper is indeed
similar to what we call guess and conquer in this work but it is only
formulated for a specific problem, not in general terms as we do, and
also not for the wide range of problems we consider; in particular,
our technique for domination and covering problems is completely
new. Additionally, their method works only for problems with a
polynomial kernel whereas we also obtain nearly subexponential
algorithms on problems without such a kernel. Furthermore, even on
problems with a kernel we obtain faster algorithms, having a running
time of $\Oof(2^{\Oof(\sqrt{k \log k})} n^{\Oof(1)})$ instead of
$\Oof(2^{\Oof(\sqrt{k} \log k)} n^{\Oof(1)})$ of~\cite{DornFLRS10}.

\usec{Odd-Minor-Free Graphs} The class of odd-minor-free graphs has
attained extensive attention in the graph theory
literature~\cite{Guenin01,GeelanGGRSV04} and recently, in theoretical
computer
science~\cite{KawarabayashiMohar06,DemaineHK10,KawarabayashiLR10}. They
are strictly more general than $H$-minor-free graphs as they include,
for example, all bipartite graphs and may contain a quadratic number
of edges. In addition to their role in graph minor theory and
structural graph theory, they bear important connections to the
$\maxcut$ problem~\cite{Guenin01} and Hadwiger's
conjecture~\cite{Hadwiger43,KawarabayashiMohar06}. We refer to the
work of Demaine et al.~\cite{DemaineHK10} for a more thorough
introduction to odd-minor-free graphs and their significance.

Demaine et al.~\cite{DemaineHK10} prove a decomposition theorem for
odd-$H$-minor-free graphs that is similar to the RS-decomposition of
$H$-minor-free graphs and present an $\Oof(n^{f(|H|)})$ algorithm to
compute such a decomposition.  From this, they derive a Baker-style
decomposition of odd-minor-free graphs into $2$ graphs of bounded
treewidth. We identify an intermediate decomposition implicit
in~\cite{DemaineHK10} that is computable in $\fpt$-time and proves to
be very useful algorithmically: on one hand, we deduce the Baker-style
decomposition into $2$ parts and a number of $2$-approximation
algorithms (most notably for \coloring) in $\fpt$-time as a corollary;
on the other hand, we can answer a question that is posed several
times by Demaine et al.\ in~\cite{DemaineHK10}, affirmatively:
nameley, whether the PTASes and subexponential $\fpt$-algorithms for
\vrtcover and \indset can be generalized from $H$-minor-free graphs to
odd-minor-free graphs. We show how to obtain such algorithms by
introducing a novel dynamic programming technique on odd-minor-free
graphs based on solving a certain weighted version of the considered
problems in bipartite graphs. These are the first PTASes and
subexponential $\fpt$-algorithms developed on odd-minor-free graphs.

\usec{Organization} We recall some relevant notions from graph theory
and parameterized complexity in Section~\ref{sect:prelim}. The
partitioning algorithm and its implications are presented in
Section~\ref{sect:hpartition}.  In Section~\ref{sect:gnc}, we state
and discuss our technique for (nearly) subexponential
$\fpt$-algorithms. Our algorithms on odd-minor-free graphs are
presented in Section~\ref{sect:oddminors} and we conclude in
Section~\ref{sect:conclusion}.


==> prelim.tex <==

\section{Preliminaries}
\label{sect:prelim}
We collect the relevant concepts from parameterized complexity and graph theory.

\usec{Subexponential Algorithms and \fpt} We use the standard notions
of parameterized complexity and bounded fixed-parameter
tractability~\cite{FlumGrohe06}.  A parameterized problem is said to
be \emph{fixed-parameter tractable} (\fpt) if for any instance of size
$n$ with parameter $k$ it can be solved in time $f(k)n^{\Oof(1)}$, for
some computable function $f$ solely dependant on $k$.  If $f$ belongs
to a class $\FFF$ of functions from $\N$ to $\N$, we say that our
problem is in $\FFF$-\fpt.  We denote $2^{k^{\Oof(1)}}$-\fpt,
$2^{\Oof(k)}$-\fpt, and $2^{\oeff(k)}$-$\fpt$ by \expt, \ept, and
\subept, respectively; here, $f \in \oeff(g)$ if there exists $n_0 \in
\N$ and a computable, nondecreasing and unbounded function $\iota: \N
\rightarrow \N$, such that $f(n) \leq \frac{g(n)}{\iota(n)}$ for all
$n \geq n_0$.  A problem is \emph{subexponential fixed-parameter
tractable} if it is in \subept.

Observe that if a problem is in $\subept$ then there exists an
algorithm for the problem, so that for any fixed $\alpha > 0$ the
algorithm runs in time $\Oof(2^{\alpha k}n^{\mathcal O(1)})$.  We
define a problem to be in $\subeptp$ if it is solved by an algorithm
$\AAA$, so that for any fixed $\alpha > 0$, the running time of $\AAA$
is $\Oof(2^{\alpha k} n^{\Oof(1/\alpha)})$.  Observe that we require a
\emph{single} (uniform) algorithm to have this property for the
considered problem.  Clearly, $\subept \subseteq \subeptp \subseteq
\ept$.  Note that the \emph{non-uniform exponential time hypothesis
(ETH)} implies that $\subeptp \neq \ept$.

\usec{Kernels} A \emph{kernel} of a parameterized problem is a fully
polynomial algorithm that given an instance of size $n$ and parameter
$k$, returns a \emph{equivalent reduced instance} of the same problem
of size $f(k)$ and parameter $k' \leq k$. The function $f$ denotes the
\emph{size} of the kernel; we then speak of a \emph{linear,
  polynomial, and subexponential} kernel, respectively. Kernelization
is a major technique in fixed parameter complexity as any computable
parameterized problem is in $\fpt$ if and only if it admits a
kernel~\cite{Niedermeier02}.

\usec{Graphs and Minors} We usually denote graphs by letters $G,H$,
and refer to their vertex/edge sets by $\vrtG$ and $\edgeG$,
respectively. Unless otherwise mentioned, our graphs have $n$ vertices
and $m$ edges. For a subset $U \subseteq \vrtG$, we write $G[U]$ to
denote the subgraph of $G$ induced by $U$. The
\emph{$r$-neighborhood} of a vertex $v$, denoted by $N_r(v)$, is the
set of vertices at distance at most $r$ from $v$; we define $N(v) =
N_1(v)$. We let $d_G(u,v)$ denote the distance between vertices $u,v
\in \vrtG$. For an edge $e=uv$ in $G$, we define the operation $G/e$
of \emph{contracting} $e$ as identifying $u$ and $v$ and removing all
loops and duplicate edges. A graph $H$ is a \emph{minor} of $G$,
written as $H \preceq G$, if it can be obtained from $G$ by a series
of vertex and edge deletions and contractions. We say $G$ is an
\emph{$H$-minor-free graph} if it does not contain $H$ as a minor. A
class of graphs that is closed under building minors and does not
contain all graphs is called a \emph{proper minor-closed class of
  graphs}. A class of graphs is a proper minor-closed class if and
only if it is $H$-minor-free for some fixed $H$. Examples of such
classes include planar graphs, bounded-genus graphs, and linklessly
embeddable graphs. An \emph{apex-graph} is a planar graph augmented by
an additional vertex that can have edges to any other vertex. A class
of graphs is called \emph{apex-minor-free} if it excludes a fixed
apex-graph as a minor. It is a well-known fact that $H$-minor-free
graphs have bounded average degree (depending only on $|H|$), i.e.\
they fulfill $m = \OHof(n)$; we use the notation $\OHof$ to denote
that the constants hidden in the big-$\Oof$ depend on
$|H|$.\footnote{this is necessary since in graph minor theory, the
  exact dependence is often not known.} We refer the reader
to~\cite{Diestel05} for more background on graph theory.

\usec{Odd Minors} A \emph{model} of $H$ in $G$ is a map that assigns
to every vertex $v$ of $H$, a connected subtree $T_v$ of $G$ such that
the images of the vertices of $H$ are all disjoint in $G$ and there is
an edge between them if there is an edge between the corresponding
vertices in $H$. A graph $H$ is a minor of $G$ if and only if $G$
contains a model of $H$. Now $H$ is an \emph{odd-minor} of $G$ if
additionally the vertices of the trees in the model of $H$ in $G$ can
be $2$-colored in such a way that (i) the edges of each tree $T_v$ are
bichormatic; and (ii) every edge $e_G$ in $G$ that connects two trees
$T_u$ and $T_v$ and corresponds to an edge $e_H=uv$ of $H$ is
monochromatic. A graph is \emph{odd-$H$-minor-free} if it excludes $H$
as an odd minor. For example, bipartite graphs are
odd-$K_3$-minor-free.

\usec{Tree Decompositions and Dynamic Programming} A \emph{tree
  decomposition} of a graph $G$ is a pair $(T,\BBB)$, where $T$ is a
tree and $\BBB=\set{B_u | u \in \vrtT}$ is a family of subsets of
$\vrtG$, called \emph{bags}, such that (i) every vertex of $G$ appears
in some bag of $\BBB$; (ii) for every edge $e=\set{u,v}$ of $G$,
there is a bag of $\BBB$ containing $\set{u,v}$; and (iii) for every
vertex $v \in \vrtG$ the set of bags containing $v$ forms a connected
subtree $T_v$ of $T$. The \emph{width} of a tree decomposition is the
maximum size of any bag in $\BBB$ minus $1$.  The \emph{treewidth} of
$G$, denoted by $\tw(G)$, is the minimum width over all possible tree
decompositions of $G$.  The \emph{adhesion} of a tree decomposition is
defined as $\max \set{|B_u \cap B_t|~|~\set{u,t} \in E_T}$.  Many
$\NP$-hard optimization problems become fixed-parameter tractable when
parameterized by the treewidth of the instance, by using dynamic
programming on a given tree decomposition.  The most well-known result
in this area is Courcelle's theorem~\cite{Courcelle90} stating that
any problem definable in monadic second-order logic is in $\fpt$ when
parameterized by the treewidth and the length of the formula.
However, the algorithms obtained by this theorem usually have
multiply-exponential dependence on the treewidth of $G$.  In this
work, we are interested in algorithms with singly-exponential
dependence on the treewidth, i.e.\ problems that are in $\ept$ when
paramterized by treewidth.  Several natural problems have long been
known to admit such
algorithms~\cite{ArnborgProskurowski89,Bodlaender88}, and for problems
with global connectivity requirement such as \longestpath,
\steiner~and \cdomset, Dorn et al.~\cite{DornFT08} recently gave
$\ept$-algorithms on (some classes of) $H$-minor-free graphs by
utilizing Catalan structures.

\usec{On Local Treewidth} We say that a graph has \emph{bounded local
  treewidth} if for every vertex $v$ and integer $r$, we have
$\tw(N_r(v)) \leq f(r)$, for some computable function $f$ depending
solely on $r$; we write $\ltw_r(G) \leq f(r)$. Demaine and
Hajiaghayi~\cite{DemaineHajiaghayi04} showed that every minor-closed
class of graphs that has bounded local treewidth has, in fact,
\emph{linear} local treewidth, i.e.\ in this case, we have $\ltw_r(G)
\leq \lambda r$ for a fixed integer $\lambda$ depending only on the
excluded minor of the class. Eppstein~\cite{Eppstein00-DT} showed that a
minor-closed class of graphs has bounded local treewidth if and only
if it is apex-minor-free.

